Measuring and mitigating voting access disparities: a study of race and polling locations in Florida and North Carolina

Voter suppression and associated racial disparities in access to voting are long-standing civil rights concerns in the United States. Barriers to voting have taken many forms over the decades. A history of violent explicit discouragement has shifted to more subtle access limitations that can include long lines and wait times, long travel times to reach a polling station, and other logistical barriers to voting. Our focus in this work is on quantifying disparities in voting access pertaining to the overall time-to-vote, and how they could be remedied via a better choice of polling location or provisioning more sites where voters can cast ballots. However, appropriately calibrating access disparities is difficult because of the need to account for factors such as population density and different community expectations for reasonable travel times. In this paper, we quantify access to polling locations, developing a methodology for the calibrated measurement of racial disparities in polling location "load" and distance to polling locations. We apply this methodology to a study of real-world data from Florida and North Carolina to identify disparities in voting access from the 2020 election. We also introduce algorithms, with modifications to handle scale, that can reduce these disparities by suggesting new polling locations from a given list of identified public locations (including schools and libraries). Applying these algorithms on the 2020 election location data also helps to expose and explore tradeoffs between the cost of allocating more polling locations and the potential impact on access disparities. The developed voting access measurement methodology and algorithmic remediation technique is a first step in better polling location assignment.

==> lp-kmedian.tex <==

\subsection{Fairness using standard clustering methods}
\label{sec:algor-fair-clust}

Sections~\ref{sec:lp} and~\ref{sec:facloc} will present algorithms for fair clustering  under the measures of fairness introduced above. Before that, we make a simple observation about approximation guarantees we can achieve by using standard clustering algorithms with minor modification. % without any consideration of group structure or fairness. 

If our data $X$ is composed of groups $X_1, X_2, \dots, X_m$ as we discussed, then optimizing the cost function on $X$ would correspond to the minimization problem:
\[\min_C \sum_{i \in X_i} \cost_{C}(X_i). \]

For most known cost functions and algorithms, it turns out that adding a {\em weight} for each point still allows for efficient algorithms. Let us consider assigning a weight of $1/|X_i|$ to all the points in $X_i$. Then the weighted minimization problem is
\begin{equation}
\min_C \sum_{i \in X_i} \frac{1}{|X_i|} \cost_{C}(X_i).\label{eq:weighted-problem}
\end{equation}

The observation is now the following.
\begin{obs}
Let $C$ be a clustering produced by an $\alpha$-approximation algorithm for the problem~\eqref{eq:weighted-problem}.  Then $C$ achieves an $\alpha m$ approximation to the fair clustering problem (definition~\ref{def:fair}) with the same cost function.
\label{obs:simple}
\end{obs}
\begin{proof}
Let $\Theta$ be the objective value for the fair clustering problem, and let $C^*$ be the corresponding clustering. Then by definition, we have
\[ \max_i \frac{1}{|X_i|} \cost_{C^*} (X_i) = \Theta \implies \sum_i \frac{1}{|X_i|} \cost_{C^*} (X_i) \le m \Theta.\]
Because the solution found by the algorithm ($C$) is an $\alpha$ approximation, we have that
\[ \sum_i \frac{1}{|X_i|} \cost_{C} (X_i) \le \alpha \cdot \sum_i \frac{1}{|X_i|} \cost_{C^*} (X_i) \le m\Theta. \]
This implies that each term is $\le m\Theta$, implying the desired approximation bound.
\end{proof}

This observation implies, for example, that for the fair versions of $k$-means and $k$-median, we can use known constant factor approximation algorithms to get $O(m)$ factor approximation algorithms directly.

%Recall that the $k$-median problem asks for a clustering that minimizes the (weighted) sum of distances from points to the closest of $k$ centers. 


%All the standard algorithms for the unconstrained $k$-median problem can be modified to incorporate weights on the points (which are used to weight the distances of points to their nearest center in the objective). Suppose we set the weight of each point in $X_i$ to $1/|X_i|$. Then the observation follows by observing that at least one of the groups must contribute a cost that is at least a $1/m$ fraction of the optimal cost solution, and therefore the \error-fair clustering cost must be at least $\frac{1}{m} \cdot \cost_C(X)$. 

\iffalse
\begin{obs}
Consider an arbitrary clustering algorithm and a set of data points $X$ comprised of $m$ demographic groups $X_i, i \in \{1, \dots,m\}$. If in the optimal standard clustering for the entire set, the largest average cost is for group $X_w$, the total $\error$ of fair clustering would not be larger than $\frac{|X|}{|X_w|}$ times the optimal solution.
\label{ob:fair-approx}
\end{obs}
\begin{proof}
Let us denote the fair clustering by $f(X)$. By assumption, the average costs for every group in $f(X)$, is no larger than the average cost for group $X_w$ in $\opt(X)$:
\[\frac{1}{|X_i|}\cost_{f(X)}(X_i) \leq \frac{1}{|X_w|}\cost_{\opt(X)}(X_w), \forall i \in \{1, \dots, m\}\]
Therefore:
\begin{align*}
\cost_{f(X)}(X) &= \sum_{i \in \{1, \dots, m\}}\cost_{f(X)}(X_i) \\
& \leq \sum_{i \in \{1, \dots, m\}}\frac{|X_i|}{|X_w|}\cost_{\opt(X)}(X_w) \\ 
& \leq \frac{|X|}{|X_w|}\cost_{\opt(X)}(X)
\end{align*}
\end{proof}
\fi

\iffalse
\maerror{Can we refer to the example in the appendix? that way we can omit the linear $j$-subspace $k$-clustering stuff too.}
We now show the analysis in theorem \ref{th:fair-approx} is tight for all variations of fair clustering introduced in section \ref{sec:notions}. Consider the relaxed version of the $k$-means problem, namely linear $j$-subspace $k$-clustering. In this problem, the goal is to find $k$ subspaces of rank at most $j$, which minimize the sum of squared distances between input points and subspaces \citep{turning,cohen}. The cost of clustering in this problem is the minimum cost of projecting data points on such subspaces. We first build the example for fair clustering, having \error as the cost function, and later make a small adjustment for it to be applicable to \Ratio{}-fair clustering as well. 

Consider minimizing the maximum cost for two groups $A$ and $B$ in Figure \ref{fig:loss-bound}, using one cluster center (here, the cluster center is 1 dimensional or simply a direction). Let's assume there are two points in each group and $r_1 \ll r_2$. Since $r_1 < r_2$, an optimal clustering with no fairness constraint would pick $x$ axis as subspace where the average \error for group $A$ is zero and the average \error for group $B$ is $r_1$. However, it is easy to see that in order to minimize the maximum average \error over both groups, we should pick $c_f$ as the fair subspace. Referring to Theorem \ref{ob:equal}, we know the average \error for the two groups is equal.\footnote{Theorem \ref{ob:equal} applies here because Frobenius norm is convex.} Therefore:
\[r_1 cos(\theta) = r_2 sin(\theta)\]
$\theta$ is inversely related to $\frac{r_2}{r_1}$. As a result, by increasing $\frac{r_2}{r_1}$, the average cost of projecting group $B$ onto the fair solution ($c_f$) gets arbitrarily close to the corresponding cost in the optimal solution ($x$ axis). Therefore, the cost of projection for all points in the fair solution would asymptotically get close to $\frac{|A|+|B|}{|B|}$ times the corresponding cost in the optimal unconstrained solution.\footnote{We should note that since the optimal cost for each group is zero, the same reasoning applies if \Loss is used as cost function}

The example above could be used to prove the tightness of the analysis in Theorem \ref{th:fair-approx} for \Ratio{}-fair clustering. However, since division by zero is not defined, we make a small adjustment. So, instead of having two points for each group, we consider two sets of points i.e. the points $A_1, A_2, B_1$ and $B_2$ in the \error{}-fair example, all become centers for points belonging to the same group. We assume these points are close enough to centers so their within group distances are negligible. The rest of the analysis is the same as before.

\begin{figure*}
\centering
\includegraphics[width=0.6\textwidth]{loss-bound.pdf}
\caption
{Minimizing the maximum average \error, provides a solution which is $1 + \frac{|A|}{|B|}$ times the optimal solution.}
\label{fig:loss-bound}
\end{figure*}

According to the result above, it may seem that different measures all have similar behavior on different data sets. However, The examples provided in Figure \ref{fig:notions}, showcase how different measures of representation cost induce different clusterings for the linear $j$-subspace $k$-clustering problem.

\begin{figure*}
        \centering
        \begin{subfigure}[b]{.6\columnwidth}
            \includegraphics[width=\textwidth]{equal-groups.png}
            \caption
            {{\small $|A| \approx |B|, cost_{opt}(A) \approx cost_{opt}(B)$}}    
            \label{}
        \end{subfigure}
        \quad
        \begin{subfigure}[b]{0.6\columnwidth}  
            \includegraphics[width=\textwidth]{different-optimal.png}
            \caption
            {{\small $|A| \approx |B|, cost_{opt}(A) \ll cost_{opt}(B)$}}    
            \label{}
        \end{subfigure}
        \\
        \begin{subfigure}[b]{0.6\columnwidth}   
            \includegraphics[width=\textwidth]{different-size_2.png}
            \caption
            {{\small $|A| \gg |B|, cost_{opt}(A) \approx cost_{opt}(B)$}}    
            \label{}
        \end{subfigure}
        \quad
        \begin{subfigure}[b]{0.6\columnwidth}   
            \includegraphics[width=\textwidth]{different-dist_2.png}
            \caption
            {{\small $|A| \approx |B|, cost_{opt}(A) > cost_{opt}(B) \approx 0$ }}    
            \label{}
        \end{subfigure}
        \caption{Comparing different fairness constraints and their induced clusterings. \error, \Ratio\Loss are shortened to AE, RE and RED respectively.}
        \label{fig:notions}
    \end{figure*} 

\sverror{this figure should be removed}
\fi 

\section{Approximation algorithms for fair $k$-clustering}\label{sec:lp}
For the fair $k$-median and $k$-means problem, we now develop approximation algorithms by writing down a linear programming relaxation and developing a rounding algorithm.

\newcommand{\lpk}{\textsc{FairLP-\error}}
\newcommand{\lpratio}{\textsc{FairLP-\Ratio}}
\newcommand{\kmed}{\textsc{K-Med-Approx}}
\newcommand{\eps}{\epsilon}
\newcommand{\cI}{\mathcal{I}}

\subsection{Relaxation for \error{}-Fair clustering}\label{sec:lp-error}
We start by considering the $\error{}$ objective for fair clustering (definitions~\ref{def:fair} and~\ref{def:abs-error}). To recap, we have a set of points $X$ that is composed of $m$ (disjoint) groups, $X_1, X_2, \dots, X_m$. We first describe the algorithm for $k$-median, and then discuss how to adapt it to the $k$-means objective (see Remark~\ref{remark:kmeans}). 

At a high level, the algorithm aims to ``open'' a subset of the $X$ as centers, and assign the rest of the points to the closest open point. The choice of the points as well as the assignment is done by using a linear programming (LP) relaxation for the problem, and rounding the obtained solution.  The variables of the LP are as follows: for $u,v \in X$,  $z_{uv}$ is intended to denote if point $u$ is assigned to center $v$. These are called assignment variables. We also have variables $y_v$ that are intended to denote if $v$ is chosen as one of the centers (or medians).  The LP (called \lpk{}) is now the following:

\begin{align}
 \min  ~\lambda \quad & \text{ subject to} \notag\\  
\begin{aligned}
\sum_v z_{uv} &= 1 \quad \text{for all $u$}, \notag \\
z_{uv} &\le y_v \quad \text{for all $u,v$}, \notag \\
\end{aligned}
&\qquad
\begin{aligned}
  \sum_{v \in X} y_v &\le k, \notag\\
0 \le z_{uv},  ~y_v &\le 1 \quad \text{for all $u, v$}.\notag \\
\end{aligned}\\
  \frac{1}{|X_i|} \cdot \sum_{u \in X_i} \sum_{v \in X} d(u, v) z_{uv} &\le \lambda \quad \text{for all groups $i$}, 
\label{eq:class-bound}
\end{align}

The only new constraint compared to the standard LP formulation for $k$-median (e.g.,~\cite{charikar2002constant}) is the constraint for all groups $i$, Eq.~\eqref{eq:class-bound}. This is to ensure that we minimize the maximum $k$-median objective over the groups. %To handle $k$-means clustering, it suffices to replace $d(u,v)$ in the constraint with $d(u,v)^2$. See Remark~\ref{remark:kmeans} for details.

\begin{thm}\label{thm:igap}
The integrality gap of \lpk{} is $\ge m$.
\end{thm}
\begin{proof}
Consider an instance in which we have $m$ groups, each consisting of a single point. Formally, let $X_i = \{x_i\}$ for all $i \in [m]$. Suppose that $d(x_i, x_j) = D$ for all $i \ne j$, and let $k=m-1$.

Now, consider the fractional solution in which $y_i = 1-\frac{1}{m}$ for all $i$. Also, let $z_{ii} = 1-\frac{1}{m}$, and let $z_{ij} = 1/m$ for some $j \ne i$ (it does not matter which one). It is easy to see that this solution satisfies all the constraints. Moreover, the LP objective value is $\lambda = D/m$.

However, in any integral solution, one of the points is not chosen as a center, and thus the objective value is at least $D$. Thus the integrality gap is $\ge m$.
\end{proof}

Theorem~\ref{thm:igap} makes it difficult for an LP based approach to give an approximation factor better than $m$ (which is easy to obtain as we saw in Observation~\ref{obs:simple}. %via a simple algorithm that finds an approximate $k$-median solution on $X$ using the weight $1/|X_i|$ for all points in $X_i$). 
However, the LP can still be used to obtain a ``bi-criteria'' approximation, where we obtain a constant approximation to the objective, while opening slightly more than $k$ clusters. 

\begin{thm}\label{thm:bicriteria}
Consider a feasible solution $(z, y)$ for \lpk{} with objective value $\lambda$.  For any $\eps > 0$, there is a rounding algorithm that produces an integral solution $(\zbar, \ybar)$ such that $\sum_v \ybar_v \le k/(1-\eps)$, all other constraints of the LP are satisfied, and the objective value is $\le 2\lambda/\eps$.
\end{thm}

There has been extensive literature on the problem of rounding LPs for problems like $k$-median (see, e.g.,~\cite{li2016approximating}). However, due to our additional fairness condition, we are interested in rounding schemes with an additional property, that we define below.

\begin{defn}[Faithful rounding]\label{def:faithful}
A rounding procedure for \lpk{} is said to be $\alpha$-faithful if it takes a fractional solution $(z, y)$ and produces an integral solution $(\hat{z}, \hat{y})$ with the guarantee that for \emph{every} $u \in X$, 
\[ \sum_{v \in X} d(u,v)~ \hat{z}_{uv} \le \alpha \cdot \sum_{v \in X} d(u,v) ~z_{uv}.\]
A weaker notion that holds for some known rounding schemes is the following: a rounding algorithm is said to be \emph{$\alpha$-faithful in expectation} if
\[ \mathbb{E} \left[ \sum_{v \in X} d(u,v)~ \hat{z}_{uv} \right] \le \alpha \cdot \sum_{v \in X} d(u,v) ~z_{uv}.\]
\end{defn}

The advantage of having a faithful rounding procedure is that it automatically gives a per-group (indeed, a per-point) guarantee on the objective value, which enables us to prove the desired approximation bound.

\begin{proof}[Proof of Theorem~\ref{thm:bicriteria}]
The proof is based on the well-known ``filtering'' technique (\cite{Lin1992approximation, charikar2002constant}). Define $R_u$ to be the {\em fractional connection cost} for the point $u$, formally, $R_u = \sum_v d(u,v) ~z_{uv}$.
Now, construct a subset $S$ of the points $X$ as follows. Set $S = \emptyset$ and $T=X$ to begin with, and in every step, find $u \in T$ that has the smallest $R_u$ value (breaking ties arbitrarily) and add it to $S$. Then, remove all $v$ such that $d(u, v) \le 2R_v / \eps$ from the set $T$. Suppose we continue this process until $T$ is empty.

The set $S$ obtained satisfies the following property: for all $u, v \in S$, $d(u, v) \ge (2/\eps) \cdot \max \{R_u, R_v\}$. This is true because if $u$ was added to $S$ before $v$, then $R_u \le R_v$, and further, $v$ should not have been removed from $T$, which gives the desired bound. The property above implies that the set of metric balls $\{ B(u, R_u/\eps) \}_{u \in S}$ are all disjoint. 

Next, we observe that each such ball contains a fractional $y$-value (in the original LP solution) of at least $(1-\eps)$.  This is by a simple application of Markov's inequality. By definition,
$R_u = \sum_{v} d(u, v) ~z_{uv}$, and thus $\sum_{v \not\in B(u, R_u/\eps)} z_{uv} \le \eps$. This means that $\sum_{v \in B(u, R_u/\eps)} x_{uv} \ge 1-\eps$, and thus $\sum_{v \in B(u, R_u/\eps)} y_v \ge 1-\eps$. As the balls are disjoint, we have that $|S| \le k/(1-\eps)$. 

Now, consider an algorithm that opens all the points of $S$ as centers. By construction, all $v \not\in S$ are at a distance $\le 2R_v/\eps$ from some point in $S$, and thus for any group $i$, we have that 
$\sum_{u \in X_i} d(u, S) \le \sum_{u \in X_i} 2R_u/\eps \le 2\lambda/\eps$. Setting $\ybar$ to be the indicator vector for $S$ and $\zbar$ to be the assignment mapping each point to the closest neighbor in $S$, the theorem follows.
\end{proof} 

\begin{remark}[Extension to $k$-means]\label{remark:kmeans}
The argument above can be extended easily to obtain similar results for the $k$-means objective. We simply replace all distances with the squared distances. The metric ball around each point can be replaced with the $\ell_2^2$ ball, and the same approximation factors can be shown to hold.
\end{remark}

\paragraph{Beyond bi-criteria: an LP based heuristic.} While Theorem~\ref{thm:bicriteria} can achieve $\sum \ybar_v = k/(1-\eps)$ for any $\eps >0$, it is still weaker than what is possible for the standard $k$-median problem. The integrality gap instance shows that this is unavoidable in the worst case (using this LP). % the factor $m$ integrality gap is special in the sense that every group has exactly one point, and thus it is impossible for an integer solution with $k=(m-1)$ to achieve a small cost for all of them.  
However, it turns out that there exist rounding algorithms for $k$-median that are faithful in expectation (as in Definition~\ref{def:faithful}), and end up with $\sum \ybar_v$ being precisely $k$. Specifically,
\begin{thm}[\cite{charikar2012dependent}]\label{thm:charikar-li}
There exists a rounding algorithm for \lpk{} that is $\alpha$-faithful in expectation with $\alpha \le 4$, and outputs precisely $k$ clusters.
\end{thm}

%The proof uses a dependent rounding (see~\cite{Chekuri2010dependent, Srinivasan2001distributions}) procedure. We note that some of the other LP rounding schemes (e.g.,~\cite{charikar2002constant}) are not faithful. Formally,


\begin{corr}
\label{corr:faithful}
Let $(z, y)$ be a solution to $\lpk{}$. There exists a rounding algorithm that (a) produces precisely $k$ clusters, and (b) ensures that the expected connection cost for every group is $\le 4 \lambda$.
\end{corr}
The corollary follows directly from Theorem~\ref{thm:charikar-li}, by linearity of expectation. This does not guarantee that the rounding {\em simultaneously} produces a small connection cost for all groups, but it gives a good heuristic rounding algorithm. In examples where every group has many points well-distributed across clusters, the costs tend to be concentrated around the expectation, leading to small connection costs for all clusters. We will see this via examples in the experiments section \ref{sec:experiment-kmedian}.

\subsection{Relaxation for \Ratio{}-Fair clustering}\label{sec:lp-ratio}
We now show that the rounding methods introduced in Section~\ref{sec:lp-error} can also be used for \Ratio{}-fair clustering. We consider the following auxiliary LP:% However, the LP in this case is not quite a relaxation:

\begin{align}
\min~\lambda \quad &\text{ subject to} \notag\\  
\begin{aligned}
\sum_v z_{uv} &= 1 \quad \text{for all $u$}, \notag \\
z_{uv} &\le y_v \quad \text{for all $u,v$}, \notag \\
\end{aligned}&\qquad
  \begin{aligned}
\sum_{v \in X} y_v &\le k, \notag\\    
0 \le z_{uv},  ~y_v &\le 1 \quad \text{for all $u, v$},\notag\\
\end{aligned}\\
\sum_{u \in X_i} \sum_{v \in X} d(u, v) z_{uv} &\le \lambda \cdot \kmed (X_i) \text{ for all $i$.}
\label{eq:class-bound-ratio}
\end{align}
The constraint~\eqref{eq:class-bound-ratio} now involves a new term, $\kmed (X_i)$, which is an approximation to the optimum $k$-median objective of the set $X_i$.  For our purposes, we do not care how this approximation is achieved --- it can be via an LP relaxation~\cite{charikar2002constant, Li2013approximating}, local search~\cite{arya2004local, gupta2008}, or any other method.  We assume that if $\vartheta_i$ is the optimum $k$-median objective for $X_i$, then for all $i$, $\frac{\kmed(X_i)}{\vartheta_i} \le \rho$ for some constant $\rho$. (From the works above, we can even think of $\rho$ as being $\le 3$.)

\begin{lemma}\label{lem:ratio-approx}
Suppose there is a rounding procedure that takes a solution $(\lambda, z, y)$ to \lpratio{} and outputs a set of centers $S$ with the property that for some parameter $\eta$, 
\begin{equation}
\label{eq:ratio-class-bound} \sum_{u \in X_i} d(u, S) \le \eta \lambda \cdot \kmed(X_i) \quad \text{for all groups $i$}.
\end{equation}
Then, this algorithm provides an $\eta \cdot \rho$ approximation to \Ratio{}-fair clustering.
\end{lemma}
\begin{proof}
Let $\opt$ be the optimum value of the ratio-fair objective on the instance $\{X_1, \dots, X_m\}$.  The main observation is that the LP provides a lower bound on $\opt$. This is true because any solution to ratio-fair clustering leads to a feasible integral solution to \lpratio{}, where the RHS of the constraint~\eqref{eq:class-bound-ratio} is replaced by $\lambda \cdot \vartheta_i$.  Since $\vartheta_i \le \kmed(X_i)$, it is also feasible for \lpratio{}, showing that the optimum LP value is $\le \opt$.

Next, consider a rounding algorithm that takes the optimum LP solution $(\lambda^*, z^*, y^*)$ and produces a set $S$ that satisfies~\eqref{eq:ratio-class-bound} (with $\lambda^*$ replacing $\lambda$ on the RHS). Then, since $\kmed(X_i) \le \rho \vartheta_i$, we have
\[ \sum_{u \in X_i} d(u, S) \le (\rho \eta) \lambda^* \cdot \vartheta_i \quad \text{for all groups $i$},\]
and using $\lambda^* \le \opt$ completes the proof of the lemma.
\end{proof}

Thus, it suffices to develop a rounding procedure for \lpratio{} that satisfies~\eqref{eq:ratio-class-bound}. Here, we observe that the rounding from Theorem~\ref{thm:bicriteria} directly applies (because ensures that every $u \in X$, $d(u, S) \le 2 R_u/\epsilon$), giving us the same bi-criteria guarantee (and the same adjustment under faithful rounding). 

\begin{corr}[Corollary to Theorem~\ref{thm:bicriteria}]\label{corr:ratio}
For any $\eps>0$, there is an efficient algorithm that outputs $k/(1-\eps)$ clusters and achieves a $(6/\eps)$ approximation to the optimum  value of the \Ratio{} objective.
\end{corr}

% Once again, we note that any faithful rounding scheme provides a good LP-based heuristic that can potentially open precisely $k$ centers (as opposed to $k/(1-\eps)$ in Corollary~\ref{corr:ratio}).


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "clustering"
%%% End:


==> ls-bad-eg.tex <==
Unlike the LP-Fair $K$-Medians, we do not provide any theoretical bounds on LS-Fair $K$-Median. In fact, the following example shows that LS-Fair $K$-Medians algorithm with the \error{}-fair objective can have local optima that are arbitrarily worse than the global optimum.

\paragraph{Description of the instance.} Let $A$ and $B$ two sets that are far apart (think of the distance between any pair as $M \rightarrow \infty$). $A = A_1 \cup A_2$, where $|A_1| = 1$ and $|A_2| = t$, for some integer parameter $t$. Likewise, suppose that $B = B_1 \cup B_2$, of sizes $1, t$ respectively. Suppose that all the elements of $A_2$ (so also $B_2$) are at distance $\eps$ away from one another. Suppose the distance between $A_1$ and $A_2$ (so also $B_1$ and $B_2$) is $d$. 

Now, suppose the two groups are $X_1 = A_1 \cup B_2$ and $X_2 = B_1 \cup A_2$.  Let $k=2$. The optimal solution is to choose one point in $A_2$ and another in $B_2$.  This results in an objective value of
\[ \max \{ t \eps + d, t\eps + d \} = t\eps +d. \]

Consider the solution $\{a_1, b_1\}$ that chooses the unique points from $A_1$ and $B_1$. The $k$-median objective for both the groups is $td$, and thus the \error{}-fair objective is $td$.  Now, consider swapping $a_1$ with some point $x \in A_2$. This changes the $k$-median objective for group 1 from $td$ to $td+\eps$, and so even though the swap significantly decreases the objective for the second group, the local search algorithm will not perform the swap. The same argument holds for swapping $b_1$ with a point $y \in B_2$. It is thus easy to see that $\{a_1, b_1\}$ is a locally optimum solution.

However, the ratio between the \error{}-fair objectives of this solution and the optimum is $\frac{td}{t \eps + d} \approx t$ for $\eps \rightarrow 0$. Thus the gap can be as bad as the number of points.


==> related.tex <==
\section{Related Work}

\sffatal{This needs to be expanded (or reintegrated and this section cut}

